JSJ decomposition for handlebody-knots

The paper applies the JSJ decomposition and Koda-Ozawa's annulus classification to analyze the annulus configuration in a handlebody-knot exterior. We introduce the notion of the annulus diagram, to pack the configuration into a labeled graph, and classify genus two handlebody-knots in terms of their annulus diagrams. Applications to handlebody-knot symmetries are discussed; methods to produce handlebody-knots with various types of annulus diagrams are also presented.

==> looping.tex <==

\subsection{Atoroidal spatial graphs}
A spatial graph is called atoroidal if 
its exterior is atoroidal. Throughout the 
section, all spatial graphs are assumed to be atoroidal. 
Atoroidal $\theta$-graphs (resp.\ handcuff graphs) 
can be classified into four types based on
their constituent knots (resp.\ links). 

Recall that a spatial graph is said to be 
minimally knotted 
if it is not planar but all its constituent knots 
and links are planar; 
given a knot $\pairk$ (resp.\ a link $\pairl$) 
and a joining arc $\tau$ of $K$ (resp. $L$) 
is an arc in $\sphere$
with $\tau\cap K=\partial \tau$ (resp.\ $\tau\cap L=\partial \tau$ and $\tau\cup L$ connected), we say $\tau$ is a 
tunnel of $K$ (resp.\ $L$) if $\pairNktau$ (resp.\ $\pairNltau$)
is trivial; otherwise, we say $\tau$ is 
a knotting arc of $K$ (resp.\ $L$). Note that
by Lemma \ref{lm:tri_redu_toro}, 
$\tau$ is the latter if and only if 
$\pairNktau$ (resp.\ $\pairNltau$) is irreducible.
Given a $2$-component split link $\pairl$, a joining arc $\tau$
is trivial if there exists a $2$-sphere $\Stwo$ 
in $\sphere$ such that $L\cap\Stwo$ is a point.


\begin{definition}
Given 
%an atoroidal 
a spatial $\theta$-graph $\pairSG$,
we say it is of
\begin{itemize}
\item type $\tht1$ if $\pairSG$ is planar;
\item type $\tht2$ if $\pairSG$ is minimally knotted;
%all constituent knots of 
%$\pairSG$ are trivial 
%and $\pairNSG$ is irreducible;
\item type $\tht3$ if $\pairSG$ is a union of a non-trivial knot
with a tunnel;
\item type $\tht4$ if $\pairSG$ is a union of a non-trivial knot
with a knotting arc.
\end{itemize}
\end{definition}

\begin{proposition}\label{prop:classification_atoro_theta}
Given an atoroidal $\theta$-graph $\pairSG$,
then it is of type $\tht1$, $\tht2$, $\tht3$ or $\tht4$.  
\end{proposition}
\begin{proof}
It follows from the definitions
of minimally knotted spatial graphs and
knotting arcs of a knot.
\end{proof}

%In the case $\pairSG$ is atoroidal,
We have the following alternative
characterization of types $\tht2$ and $\tht4$ atoroidal spatial $\theta$-graphs more relevant to the construction of handlebody-knots.
\begin{lemma}\label{lm:irre_typeII_IV_theta}
Let $\pairSG$ be an atoroidal spatial $\theta$-graph.
Then it is of type $\tht2$ or type $\tht4$ if and only if 
$\pairNSG$ is irreducible.
\end{lemma}
%add proof
\begin{proof}
``$\Leftarrow$'': If it is of type $\tht1$ or type $\tht3$,
then $\pairNSG$ is trivial and hence reducible.

``$\Rightarrow$'': By Lemma \ref{lm:tri_redu_toro},
if $\pairNSG$ is reducible, it is trivial.  
If there exists a non-trivial constituent knot
in $\pairSG$, then it is of type $\tht3$;
otherwise by the unknotting theorem
\cite{SimWol:90}, \cite{SchTho:91}, 
it is planar and hence of type $\tht1$.
\end{proof}
\cout{
Suppose all constituent knots of $\pairSG$ 
are trivial. Then 
by the unknotting theorem 
\cite{SimWol:90}, \cite{SchTho:91}, 
$\pi_1(\Compl\SG)$ is free if and only if 
$\pairSG$ is planar; on the other hand,
by Lemma \ref{lm:tri_redu_toro}, 
$\pairNSG$ is not trivial
if and only if $\pairNSG$ is irreducible,
so $\pairSG$ is either of type I or of type II.

Suppose some constituent knot $\pairk$ of $\pairSG$ is non-trivial. Then the arc $\tau:=\overline{\SG-K}$
is either a tunnel or a knotting arc of $K$, depending on
whether $\pairNSG$ is trivial. 
}


\begin{definition}
Let $\pairSG$ be an atoroidal spatial handcuff graph $\pairSG$; denote by $L$ its constituent link, and $\tau\subset\SG$ its joining arc. 
Then we say it is of
\begin{itemize}
\item type $\hc1$ if $\pairSG$ is planar;
\item type $\hc2$ if $\pairl$ is split and $\tau$ is non-trivial;
%all constituent knots of 
%$\pairSG$ are trivial 
%and $\pairNSG$ is irreducible;
\item type $\hc3$ if $\pairl$ is non-split and $\tau$ is a tunnel;
\item type $\hc4$ if $\pairl$ is non-split and $\tau$ is a knotting arc.
\end{itemize}
\end{definition}

\begin{proposition}\label{prop:classification_atoro_handcuff}
Given an atoroidal handcuff graph $\pairSG$,
then it is of type $\hc1$, $\hc2$, $\hc3$ or $\hc4$.  
\end{proposition}
\begin{proof}
It is clear that if $\pairl$ is non-split $\pairSG$
is either of type $\hc3$ or type $\hc4$. 
On the other hand, $\pairSG$
is always toroidal in the case $\pairl$ is non-trivial split link
with $\tau$ a trivial joining arc, so if $\pairl$ is split, 
$\pairSG$ is either of type $\hc1$ or of type $\hc2$.
\end{proof}

\begin{lemma}\label{lm:irre_typeII_IV_handcuff}
Let $\pairSG$ be an atoroidal spatial handcuff graph.
Then it is of type $\hc2$ or $\hc4$ if and only if 
$\pairNSG$ is irreducible.
\end{lemma}
\begin{proof}
``$\Leftarrow$'': If it is of type $\hc1$ or $\hc3$,
then $\pairNSG$ is trivial and hence reducible.

``$\Rightarrow$'': If $\pairNSG$ is reducible, 
it is trivial by Lemma \ref{lm:tri_redu_toro}.
Therefore it is of type $\hc3$ if $\pairl$ is non-split.
Now, observe that if 
$\pairl$ is split and non-trivial,
then the rank of $\pi_1(\Compl L)$ is at least $3$;
on the other hand if $\tau$ is a tunnel, it implies
$\pi_1(\Compl L)$ is of rank $2$. Thus $\pairl$
has to be trivial. By the unknotting theorem
\cite{SimWol:90}, \cite{SchTho:91}, this implies 
$\pairSG$ is planar and therefore of type $\hc1$.
\end{proof}

\subsection{The looping operation}
Here we introduce a construction that produces 
an irreducible, atoroidal handlebody-knot 
whose exterior contains a 
type $2$ annulus from a spatial 
$\theta$-graph or handcuff graph.

Let $\Gamma$ be a spatial $\theta$-graph 
%whose exterior 
%$\Compl\Gamma_0$ is atoroidal, 
and $\alpha,e,f$ be   
a trivalent node and two edges in $\Gamma$, respectively. 
Then we construct the spatial handcuff graph $(\sphere,\Gamma_{\alpha,e,f})$ as follows:
choose a small regular neighborhood $\rnbhd \alpha$ 
of $\alpha$ so that $\big(\rnbhd\alpha, \partial\rnbhd\alpha\cap d, \rnbhd\alpha\cap (e\cup f)\big)$ is homeomorphic to 
the triplet $\big(B^3, (1,0,0), B^3\cap \{x=y=0\}\big)$,
where $d$ is the other edge of $\Gamma$ and 
$B^3$ is the unit $3$-ball in $\mathbb{R}^3$;
then define the spatial handcuff graph 
$\Gamma_{\alpha,ef}$ in $\sphere$
to be the union 
\[
(\Gamma-\openrnbhd\alpha)\cup f^{-1}\big(\{(x,y,0)\mid x^2+y^2=1\}\big)\subset \sphere,
\]
where $f$ is the homeomorphism 
\[\big(\rnbhd\alpha, \partial\rnbhd\alpha\cap d, \rnbhd\alpha \cap (e \cup f)\big)\rightarrow 
\big(B^3, (1,0,0), B^3\cap \{x=y=0\}\big).
\]
The construction depends only on $\alpha,e, f$,
and $(\sphere,\Gamma_{\alpha,e,f})$ 
is said to a looping of $\pairSG$ 
obtained by ``looping $ef$ at $\alpha$''.
When the specifications $\alpha,e,f$
are irrelevant in the discussion,
they are dropped from the notation, and 
we denote by $\pairLSG$ 
a spatial handcuff obtained from $\pairSG$ by
looping some edges at a trivalent node in $\Gamma$.

When $\Gamma$ is a union of a non-trivial knot $K$ 
and a tunnel $\tau$ in $\sphere$, 
we denote by $k_1,k_2$ the edges of $\Gamma$
that are in $K$, and say $\pairLSG$
is a \emph{tunnel looping} of $\pairSG$
if it is obtained by looping $k_1k_2$
at some trivalent node of $\Gamma$,
and say it is a \emph{knot looping}
of $\pairSG$ if it is obtained by looping 
$k_i\tau$ at some trivalent node of $\Gamma$, $i=1$ or $2$. 




Given a spatial handcuff graph 
$\Gamma$, we can perform a similar construction.
%with $\Compl\Gamma$ atoroidal. 
Choose a trivalent node $\alpha$, 
and fix an orientation of the loop $l$ containing
$\alpha$, and choose 
a small regular neighborhood $\rnbhd\alpha$ of $\alpha$ so
that $B\cap l$ is an arc and the triplet 
$\big(\rnbhd\alpha, \partial\rnbhd\alpha \cap 
l_\pm, \rnbhd\alpha \cap l_\mp\cup e \big)$ is homeomorphic to 
the triplet $\big(B^3, (1,0,0), B^3\cap \{x=y=0\}\big)$,
where $l_+$ (resp.\ $l_-$) is the closure of the complement $B\cap (l-\alpha)$
whose starting (resp.\ end) point is $\alpha$ 
with the induced orientation from $l$.

Then $\pm$-looping at $\alpha$ amounts
to replacing $(\sphere,\Gamma)$ 
with the spatial handcuff graph 
$(\sphere, \Gamma_{\alpha,\pm})$ given by 
\[
\Gamma_{\alpha,\pm}=\big((\Gamma-\openrnbhd\alpha)\cup f^{-1}(\{(x,y,0)\mid x^2+y^2=1\})\big)\subset \sphere,
\]
where $f$ is the homeomorphism identifying 
\[\big(\rnbhd\alpha, \partial\rnbhd\alpha\cap l_\pm, \rnbhd\alpha \cap (e \cup l_\mp)\big)\quad\text{with}\quad \big(B^3, (1,0,0), B^3\cap \{x=y=0\}\big).\]
The construction depends only on $\alpha$ and the
orientation of $l$; the latter is used only
to distinguish two possible loopings at $\alpha$.
When the specifications, $\alpha$ and the orientation of $l$,
are irrelevant in the presentation,
they are dropped from the notation, and 
we denote by $\pairLSG$ 
a spatial handcuff obtained by
performing the looping operation on $\SG$
at some trivalent node,
and by $\pairLHK$
the handlebody-knot 
given by taking a regular neighborhood 
$\LHK:=\rnbhd{\LSG}$ of $\LSG$. 

 
Let $\LA$ be the type $2$ annulus 
given by 
\[\LA:=f^{-1}\big(\{(x,y,0)\mid x^2+y^2\leq 1\}\big)-\openrnbhd{\LSG}.\] 
If $\SG$ is a $\theta$-graph, 
$\LA$ is of type $2$-$1$, whereas it is of type $2$-$2$
if $\LSG$ is a handcuff graph.


Conversely, consider 
an irreducible, atoroidal handlebody-knot 
$\pair$ with a type $2$ annulus $A\subset\ComplHK$.
Then $A$ induces two non-parallel disjoint disks
$D_+,D_-\subset\ComplHKA$ bounded by $l_+,l_-$, respectively.
We say a meridian disk system $\{D_1,D_2,D_3\}$
of $\HKA$ is admissible 
if it is isotopic to $\{D_+,D_-,D\}$
where $D$ is a meridian disk with $D\cap \big(D_+\cup D_-\cup A^\perp\big)=\emptyset$ and non-parallel
to $D_+,D_-$. There are infinitely many
non-isotopic admissible meridian system 
if $A$ is of type $2$-$1$; on the other hand, 
there is a
unique, up to isotopy, admissible meridian 
disk system if $A$ is of type $2$-$2$.
An admissible meridian disk system gives us
a spine $\SG_A$ of $\HKA$, and the induced spatial graph
is denoted by $\pairSGA$. 
Note that 
$\SG_A$ is a $\theta$-graph if $A$ is of type $2$-$1$,
and is a handcuff graph if $A$ is of type $2$-$2$.


The looping and annular operations are related as follows.
Let $\epsilon_\pm$ be the edges in $\SG_A$ 
dual to $D_\pm$, and $\alpha$ the trivalent node of $\SG_A$
dual to the component of $\HKA-D_+\cup D_-\cup D$
containing $A^\perp$. 
Suppose $A$ is of type $2$-$1$. Then $\pair$ 
is equivalent to the handlebody-knot
obtained by looping $\epsilon_+\epsilon_-$ at $\alpha$.
Suppose $A$ is of type $2$-$2$,
and orient $\epsilon_+$ so that starting from 
the $\alpha$, it meets $D_+$ first and then $A^\perp$.
Then $\pair$ is equivalent to the handlebody-knot obtained by
$+$ looping at $\alpha$. The spatial graph obtained 
by the looping operation described 
above is called the canonical looping of $(\sphere,\SG_A)$.



  




%onto
\begin{lemma}\label{lm:looping_surjective}
Given a handlebody-knot $\pair$ and a type $2$ annulus
$A\subset\ComplHK$, then $\pair$ 
is equivalent to the handlebody-knot $(\sphere,\HK_{\SG_A}^\odot)$ associated to the canonical looping of $\pairSGA$.
%Furthermore, if $\pair$ is irreducible and atoroidal,
%then $\pairSGA$ is atoroidal.
\end{lemma}
\begin{proof}
It follows from the construction of $\pairSGA$. 
\end{proof}
%preimage
\begin{lemma}\label{lm:looping_preimage}
Given a spatial graph $\pairSG$, if 
$\pairLHK$ is irreducible and atoroidal, then $\pairSG$
is atoroidal. In particular, $\pairSGA$ is atoroidal.
\end{lemma}
\begin{proof}
This follows from Corollary \ref{cor:atoro_HK_HKA} 
as $\pairLHKA\simeq \pairNSG$.
\end{proof}
%relation looping and contraction

%well-defined
\begin{lemma}\label{lm:looping_range}
Let $\pairSG$ be an atoroidal spatial $\theta$-graph or 
handcuff graph. 
Then any looping $\pairLSG$ of $\pairSG$  
and therefore $\pairLHK$ 
are atoroidal. 
\end{lemma}
\begin{proof}
Corollary \ref{cor:atoro_HKA_HK} implies
the assertion for the case where $\pairSG$
is a spatial $\theta$-graph or a spatial handcuff graph of
type II, III or IV. On the other hand, loops of 
a planar spatial handcuff graph always induce a trivial handlebody-knot.
\end{proof}

%a finer analysis on the effect of looping operation
From now on, in view of Lemma \ref{lm:looping_preimage},
$\pairSG$ is assumed to be atoroidal, and
unless otherwise specified, $\pair$
is assumed to be irreducible and atoroidal. 

\begin{lemma}\label{lm:looping_theta}
Let $\pairSG$ be a spatial $\theta$-graph.
Then
\begin{enumerate}[label=(\roman*)]
\item if it is of type $\tht 2$ or $\tht 4$, then any looping $\pairLSG$ is of type $\hc 4$.\label{item:looping_theta1}
\item if it is of type $\tht 1$, then $\pairLSG$ 
is equivalent to $(\sphere,2_1)$, and hence of type $\hc3$
\label{item:looping_theta2}
\item if it is of type $\tht 3$, then any knot looping
$\pairLSG$ is of type $\hc 4$.\label{item:looping_theta3}
\item if it is of type $\tht 3$, then a tunnel looping can
be of type $\hc 3$ or $\hc4$.\label{item:looping_theta4}
\end{enumerate} 
\end{lemma}

\begin{lemma}\label{lm:looping_handcuff}
Let $\pairSG$ be a spatial handcuff graph.
Then 
\begin{enumerate}[label=(\roman*)]
\item if it is of type $\hc 1$, then 
$\pairLSG$ is of type $\hc 1$.
\label{item:looping_handcuff1}
\item if it is of type $\hc 2$, $\hc 3$ or $\hc 4$, then 
$\pairLSG$ is of type $\hc 2$.
\label{item:looping_handcuff2} 
  
\end{enumerate} 
\end{lemma}

As an application of Lemmas \ref{lm:looping_theta} and \ref{lm:looping_handcuff}, we have the following.
\begin{corollary}
Given a type $\tht 2$ or $\tht 4$
(resp.\ $\hc 2$ or $\hc 4$) spatial graph 
$\pairSG$, $\pairLHK$ is irreducible, atoroidal,
and $\LA$ is essential, of type $2$-$1$ (resp.\ type $2$-$2$), and not unknotting. 

Given a type $\tht 3$ 
(resp.\ $\hc 3$) spatial graph 
$\pairSG$, the handlebody-knot $\pairLHK$
associated to a knot looping (resp.\ a looping)
is irreducible, atoroidal and $\LA$
is essential, of type $2$-$1$ (resp.\ type $2$-$2$), and
unknotting.
\end{corollary}

Conversely, we have the following as a corollary of Lemmas \ref{lm:irre_typeII_IV_theta} and \ref{lm:irre_typeII_IV_handcuff}.
\begin{corollary}
Every irreducible, atoroidal 
handlebody-knot $\pair$ with a knotting 
type $2$-$1$ (resp.\ type $2$-$2$)
annulus $A$ can be obtained by performing looping operation on
a type $\tht 2$ or $\tht 4$
(resp.\ $\hc 2$ or $\hc 4$) atoroidal spatial graph. 

Every irreducible, atoroidal 
handlebody-knot $\pair$ with an unknotting 
type $2$-$1$ (resp.\ type $2$-$2$)
can be obtained by performing tunnel looping (resp.\ performing looping) on
a type $\tht 3$ (resp.\ $\hc 3$) atoroidal spatial graph. 
\end{corollary}
\begin{proof}
Let $\pairSGA$ is an admissible spatial graph
associated to $\pair$ and $A$. 
Then Propositions \ref{prop:classification_atoro_theta} 
and \ref{prop:classification_atoro_handcuff} and Lemmas 
\ref{lm:irre_typeII_IV_theta} and \ref{lm:irre_typeII_IV_handcuff} implies that $\pairSGA$
is of $\tht2$ or $\tht 4$ (resp.\ $\hc2$ or $\hc4$)
if $\pair$ is $A$ is unknotting, and hence the first assertion.
They also imply that $\pairSGA$ is of type $\tht1$ or $\tht3$
(resp.\ $\hc1$ or $\hc3$) if $A$ is unknotting.
Since no loopings of type $\tht1$ or $\hc1$ spatial graphs
induce non-trivial handlebody-knots, $\pairSGA$
is necessarily of type $\tht3$ (resp.\ $\hc3$).

If $\pairSGA$ is of type $\tht3$, and 
$\{D_+, D_-, D\}$ is the corresponding 
admissible meridian disk system of $\HK$
associated to $A$. Denote by $\epsilon_\pm,\epsilon \subset\SG_A$
the edge dual to $D_\pm$, $D$, respectively.
Observe that one of the constituent knots 
$(\sphere, \epsilon_+\cup\epsilon)$, $(\sphere,\epsilon_-\cup\epsilon)$
is non-trivial. Suppose otherwise. Then it implies
$\ComplHKA\cup\rnbhd{D_+}$ and 
$\ComplHKA\cup\rnbhd{D_-}$ are both solid tori,
and hence by Lemma \ref{lm:primitive_surgery}, 
$\{l_+, l_-\}$ is a primitive set of loops in
the handlebody $\ComplHKA$, but this implies
$\pair$ is trivial by Lemma \ref{lm:triv_type2_1},
a contradiction. It may be assumed that
$(\sphere, K_+:=\epsilon_+\cup\epsilon)$ is non-trivial
and hence $\epsilon_-$ is a tunnel, and 
thus the canonical looping of $\Gamma_A$
is a knot looping where  
%$\pair$ is obtained by a knot looping on 
$\pairSGA$ is regarded as the non-trivial knot $(\sphere, K_+)$ with the tunnel $\epsilon_-$.   
\end{proof} 


\subsection{Double looping}
Given an atoroidal spatial graph $\pairSG$,
we say $\pairLSG$ is a double looping of $\pairSG$
if $\pairLSG$ is obtained by performing 
two looping operations on two trivalent nodes
of $\pairSG$. 
%so that the looped edges are not identical.
In the case where $\pairSG$ is a spatial $\theta$-graph,
we require that the looping operations do not loop 
identical edges on different trivalent nodes.
In particular, if $\pairSG$ is a union 
of a non-trivial knot and a tunnel,
then a double looping $\pairLSG$
can be obtained by performing either two knot looping 
or one knot and one tunnel looping
operations on the two trivalent nodes. 



Let $\pair$ be an irreducible, atoroidal handlebody-knot
whose exterior admits two type $2$-$2$ annuli $A_1,A_2$. 
Then the meridian disks $D_{i\pm}$, $i=1,2$, bounded
by $l_{i\pm}$ induce a meridian disk system $\mathcal{D}$
of $\HK_{A_1,A_2}$. Denote by $\SG_{1,2}$
the spine corresponding to $\mathcal{D}$.
Note that either $D_{1+}$, $D_{2+}$  
are parallel or $D_{1-},D_{2-}$ are parallel.
In the former, $\SG_{1,2}$ is a $\theta$-graph,
while in the the latter, $\SG_{1,2}$ 
is a handcuff graph. As with the case where $\pair$
admits one type $2$ annulus, we define 
the canonical double looping of $(\sphere,\SG_{1,2})$
to be the double looping obtained by looping 
edges dual to $D_{i\pm}$, $i=1,2$, and $\pair$ 
is equivalent to its associated handlebody-knot. 
 
\begin{lemma}\label{lm:atoroidality_core}
$(\sphere,\SG_{1,2})$ is atoroidal, and if $\pair$
is obtained by a double looping of $\pairSG$,
then $\pairSG\simeq (\sphere,\SG_{1,2})$.
\end{lemma}
\begin{proof}
If $(\sphere,\HK_{A_1})$ is irreducible,
then $(\sphere,\HK_{A_1,A_2})$ is atoroidal 
by Corollary \ref{cor:atoro_HK_HKA}. 
Suppose $(\sphere,\HK_{A_1})$
is trivial, and let $(\sphere,\SG_{A_1})$ 
be the spatial handcuff graph associated to 
the meridian disk system induced
by $D_{1\pm}$. Then $(\sphere,\SG_{A_1})$
is of type $\hc 2$ by Proposition \ref{prop:classification_atoro_handcuff} and Lemma \ref{lm:irre_typeII_IV_handcuff}. In particular,
the constituent link of $(\sphere,\SG_{A_1})$
is non-split and hence $\SG_{1,2}$ is a $\theta$-graph
and therefore $A_2$ is a type $2$-$1$ annulus in 
$\Compl{\HK_{A_1}}$; by Lemma \ref{lm:triv_type2_1},
$(\sphere, \HK_{A_1,A_2})$ is trivial and hence atoroidal.

The second assertion follows from Theorem \ref{}
as the pair $(A_1,A_2)$ is isotopic to the pair of 
type $2$-$2$ annuli obtained from the looping operations.
\end{proof}

\begin{definition}
Let $\pair$ is a handlebody-knot whose exterior contains
a type $2$-$2$ annulus. 
Then a spatial graph $\pairSG$ is called 
a core of $\pair$ if $\pair$ 
is equivalent to the associated handlebody-knot of 
a looping of $\pairSG$ when $\pair$ 
is of type $(1,1,0,\hnode)$ or $(2,1,0,\hnode)$
or of a double looping of $\pairSG$ when
$\pair$ if of type $(3,0,3,\snode)$ or $(3,0,3,\hnode)$. 
\end{definition}

\begin{lemma}
Given a handlebody-knot $\pair$ whose exterior contains
a type $2$-$2$ annulus, 
its core depends only on $\pair$.
\end{lemma}
\begin{proof}
Suppose $\pair$ is of type $(1,1,0,\hnode)$ or $(2,1,0,\hnode)$,
and $\pairSG$, $(\sphere,\SG')$ are two cores of $\pair$.
It then follows from the classification theorem \ref{} that 
there is an orientation-preserving homeomorphism
$f$ sending $\pairLHK$ to $(\sphere,\HK^\odot_{\SG'})$
with $f(\LA)=A^\odot_{\Gamma'}$. 
Thus it may be assumed that $f$ sends 
the meridian disk systems given by $\LA$
to $A^\odot_{\Gamma'}$.
The proof for the case of type $(3,0,3,\snode)$ or $(3,0,3,\hnode)$ is similar.
\end{proof}  

\begin{corollary}\label{cor:hk4_1_characterization1}
The core of $\pair$ is the planar spatial 
$\theta$-graph if and only if $\pair\simeq (\sphere,\HK4_1)$.
\end{corollary}
%core--> can we use the backbone to see uniqueness?
%discuss unknotting cases 

\begin{definition}
We say $(A_1,A_2)$ is an unknotting pair
if $\pairDA$ is trivial, and if in addition 
one of $A_1,A_2$ is unknotting, then we say it is strictly unknotting.
\end{definition}

\begin{lemma}
If $\pair$ admits an unknotting pair, then
either $\pair\simeq (\sphere,\HK4_1)$
or its core is of type $\tht 3$ or $\hc 3$.

If $\pair$ admits a strictly unknotting pair, then
either $\pair\simeq (\sphere,\HK4_1)$
or its core $\pairSG$ is of type $\tht 3$ with 
$\pair$ induced by performing a knot looping
and a tunnel looping operations on $\pairSG$.
\end{lemma}
\begin{proof}
By Lemma \ref{lm:atoroidality_core} and Propositions \ref{prop:classification_atoro_theta} and \ref{prop:classification_atoro_handcuff}, 
the core $\pairSG$ of $\pair$ is of 
type $\tht 1, \hc 1, \tht 3$ or $\hc 3$.
If it is of type $\tht 1$, 
we have $\pair\simeq (\sphere,\HK4_1)$ by Corollary \ref{cor:hk4_1_characterization1},
while if it is of type $\hc 1$, 
$\pair$ is trivial, a contradiction. 

On the other hand, if it is of type $\hc 3$ (resp.\ $\tht 3$), 
it follows from Lemmas \ref{lm:looping_theta}\ref{item:looping_theta3}, \ref{lm:looping_handcuff}\ref{item:looping_handcuff2} and \ref{lm:irre_typeII_IV_handcuff}
that any looping (resp.\ knot looping) of $\pairSG$ induces a 
non-trivial handlebody-knot,
and hence none of $A_1,A_2$ can be unknotting.
Therefore if $(A_1,A_2)$ is strictly unknotting, 
the double looping must consist of one knot and one tunnel loopings. 
\end{proof}

\begin{corollary}
$\pair$ admits a strictly unknotting pair $(A_1,A_2)$
with both $A_1,A_2$ unknotting if and only if 
$\pair\simeq (\sphere,\HK4_1)$.
\end{corollary}
\begin{proof}
``$\Leftarrow$'' is clear. 
``$\Rightarrow$'' follows from the fact
that any knot looping on a type $\tht 3$ spatial graph 
$\pairSG$
induces a non-trivial handlebody-knot; thus
if the core of $\pair$ 
is of type $\tht 3$, then one of $A_1,A_2$
is not unknotting.
\end{proof}
%try to combine the following four subsections into one
\begin{corollary}
Suppose $\pair$ admits an unknotting annulus $A$.
Then $A$ is unique if and only if $\pair\not\simeq (\sphere,\HK4_1)$.
%Let $A$ be an unknotting annulus of type $2$-$2$ in $\ComplHK$.
\end{corollary}


%Under suitable condition 
%looping construction produces irre atoro hk w type
 
%all irre atoro w type 2 is produced this way

%how is it related to tunnel of knots and 2-component link
 




==> prelim.tex <==
%%preliminaries:
%%notation
%%2-component links
 
 
Throughout the paper we work in the piecewise linear category.
Given a subpolyhedron $X$ of $M$, 
$\mathring{X}$ denotes the interior of $X$, and
%$\nbhd{X}{M}$ a regular neighborhood of $X$ in $M$, or simply
$\mathfrak{N}(X)$ a regular neighborhood of $X$ in $M$.
%when the ambient $M$ is clear from the context. 
%(e.g.\ $\opennbhd{X}{M}$).
The exterior $\Compl X$ of $X$ in $M$ is the complement of $\opennbhd{X}{M}$ if $X$ has codimension greater than zero, and  
is the closure of $M-X$ otherwise. 
Submanifolds of a manifold $M$ are 
%understood to be 
proper and in general position except in some obvious cases
where submanifolds are in $\partial M$.  
%intersection of two submanifolds are assumed to be transverse.  
A surface in a three-manifold is essential if 
it is incompressible, $\partial$-incompressible, and non-boundary parallel. We denote by $(\sphere,X)$ an embedding 
of $X$ in the oriented $3$-sphere $\sphere$. 
When $X$ is a handlebody, an essential disk in $X$ is called a \emph{meridian} disk. 
Throughout the paper $\pair$ is a handlebody-knot of genus two.
 
\begin{definition}
An annulus $A\subset\ComplHK$ 
is of type $2$ if $\partial A$ is essential in $\partial \HK$
and exactly one component of $\partial A$ 
bounds an essential disk in $\HK$. 
\end{definition}  
We denote by $\disk_A\subset\HK$ 
the disk bounded by the component of $\partial A$. 
 
\begin{definition}
A type $2$ annulus $A\subset \Compl\HK$
is of type $2$-$1$ if $\disk_A$ non-separating;
otherwise it is of type $2$-$2$.  
\end{definition}  

Note that $\pairA$ with $\HK_A=\HK\cup\rnbhd{A}$ 
is also a handlebody-knot, and we say $A$ is unknotting
if $\pairA$ is trivial.

Denote by $A_+,A_-$ the components of 
$\partial\HK_A\cap \nbhd{A}$, and $l_+,l_-$ essential loops of 
$A_+,A_-$, respectively. We orient $l_+,l_-$ so that 
they represent the same homology class in $H_1(\rnbhd{A})$.
 
\begin{lemma}
If $A$ is of type $2$-$1$, then the homology classes
$\{[l_+],[l_-]\}$ is a basis of $H_1(\ComplHKA)$.
If $A$ is of type $2$-$2$, then one of the homology classes
$[l_+], [l_-]\in H_1(\ComplHKA)$ is trivial and the other a generator. 
\end{lemma}

Let $\cl{l_+},\cl{l_-}$ be the conjugacy classes determined by 
$l_+,l_-$, respectively. 
When $A$ is unknotting, we say $\{l_+,l_-\}$ represents
a basis of $\pi_1(\ComplHKA)$ if there exist
some elements $x\in\cl{l_+},y\in\cl{l_-}$
such that $\{x,y\}$ is a basis of $\pi_1(\ComplHKA)$,
and we say $l_+$ (resp.\ $l_-$) is homotopically trivial
if $\cl{l_+}$ (resp.\ $\cl{l_-}$) contains only the identity.

\begin{lemma}
Suppose $A$ is of type $2$-$1$.
Then $\pairA$ is trivial and $\{l_+,l_-\}$ represents
a basis of $\pi_1(\ComplHKA)$ if and only if 
$\pair$ is trivial.
\end{lemma}
\begin{proof}
To see the ``only if'' part, we note that
$\pi_1(\ComplHK)$ is the HNN extension of $\ComplHKA$ with respect to $A$,
so if $\{l_+,l_-\}$ represents
a basis of $\pi_1(\ComplHKA)$, $\pi_1(\ComplHK)$ is free.

For the other direction, we observe that since 
$\ComplHK$ is a handlebody and $A$ is incompressible in $\ComplHK$,
$A$ must be $\partial$-compressible in $\ComplHK$. 
Let $D$ be a $\partial$-compressing
disk of $A$. Then $D$ induces a compressing disk $D'$ of $\partial\HK_A$
in $\ComplHKA$ that intersect with $l_+\cup l_-$ at one point.
The disk component $D''$ of $\partial \rnbhd{A\cup D'}$
is separating and disjoint from $l_+,l_-$.
Now, if $\pairA$ is not trivial, it is toroidal, but 
since $A$ is incompressible, any incompressible torus in $\ComplHKA$
is an incompressible torus in $\ComplHK$, contradicting 
$\pair$ is trivial. 

Because $\ComplHKA$ is trivial, $D''$ separates $\ComplHKA$
into two solid tori $V_1,V_2$, and by Lemma \ref{}, 
one contains $l_+$ and the other $l_-$, and neither of $l_+,l_-$
can have an non-integral slope on the respective torus. Thus
$\{l_+,l_-\}$ represents a basis of $\pi_1(\ComplHKA)$. 
\end{proof}

\begin{lemma}
Suppose $A$ is of type $2$-$2$.
Then 
$\pair$ is trivial if and only if 
$\pairA$ is trivial and one of $l_+,l_-$ is homotopically trivial.
\end{lemma} 
\begin{proof}
If $\pair$ is trivial, then $A$ is either compressible or
$\partial$-compressible. If $A$ is compressible and $D$ 
is a compressing disk, then $D$ induces an essential separating disk
$D'$ in $\ComplHKA$ which bounds an essential separating disk $D''$.
In particular, one of $l_+,l_-$ is homotopically trivial, and
$D''$ cuts $\HK_A$ into two solid tori $W_1,W_2$.
Without loss of generality, we may assume 
$l_-=\partial D''$ and hence
$l_+$ is a meridian of either $W_1$ or $W_2$.
In addition, the cores $c(W_i)$ of $W_i$, $i=1,2$ are trivial knots in $\sphere$ if and only if $\pairA$ is trivial. 
Suppose one of the cores of $W_1,W_2$ is not trivial, say $c(W_1)$.
Then $(\partial W_1-D'')\cup D'$ is an incompressible torus
in $\ComplHKA$, which is also incompressible in $\Compl\HK$. 

If $A$ is $\partial$-compressible with $D$ 
a $\partial$-compressing disk, and it may be assumed
that $D\cap l_+\neq \emptyset$,
then the disk component $D'$
of $\partial \rnbhd{D\cup A}$ is an essential separating disk 
in $\ComplHKA$ with $\partial D'$ parallel to $l_-$. 
Thus, the same argument in the preceding case implies that $\pairA$ 
is trivial.

To see the converse, we assume $l_-$ is homotopically trivial and
hence it bounds a disk $D'$ in $\ComplHKA$.
This implies $l_+$ is primitive. 
The assertion then follows from the fact that
$\pi_1(\Compl\HK)$ is the HNN-extension of $\pi_1(\ComplHKA)$
with respect to $A$.
\end{proof}
%%reducible criterion
%%a remark: non-trivial reducible => toroidal







 

